Matrix Product Density Operators: when do they have a local parent Hamiltonian?

We study whether one can write a Matrix Product Density Operator (MPDO) as the Gibbs state of a quasi-local parent Hamiltonian. We conjecture this is the case for generic MPDO and give supporting evidences. To investigate the locality of the parent Hamiltonian, we take the approach of checking whether the quantum conditional mutual information decays exponentially. The MPDO we consider are constructed from a chain of 1-input/2-output (`Y-shaped') completely-positive maps, i.e., the MPDO have a local purification. We derive an upper bound on the conditional mutual information for bistochastic channels and strictly positive channels and show that it decays exponentially if the correctable algebra of the channel is trivial. We also introduce a conjecture on a quantum data processing inequality that implies the exponential decay of the conditional mutual information for every Y-shaped channel with trivial correctable algebra. We additionally investigate a close but nonequivalent cousin: MPDO measured in a local basis. We provide sufficient conditions for the exponential decay of the conditional mutual information of the measured states and numerically confirm they are generically true for certain random MPDO.

==> letter_to_editor.tex <==
Dear Editors, 

We would like to submit our manuscript entitled ‘When do matrix-product-density-operators have a local parent Hamiltonian?’ for consideration of publication in Communications in Mathematical Physics. We certify that this submission is the original work and is not under review.


In this work, we study the conditions when a matrix product density operator (MPDO) can be regarded as the Gibbs state of some parent Hamiltonian. Tensor networks, which includes MPDO, are low dimensional ansatz to describe quantum many-body state. A triumphant case is the matrix product state (MPS). Each 1D gapped local Hamiltonian can be described by MPS and conversely each MPS is also a ground state of some parent Hamiltonian. This correspondence between MPS and its parent Hamiltonian establishes a deep connection with gapped quantum systems, leading to the complete classification of 1D gapped quantum phases. For this work, MPDO is the mixed state version of MPS, and analogously the Gibbs state of each 1D gapped local Hamiltonian was known to be described by some MPDO. Unfortunately for the converse, the renormalization procedure to simplify MPS to a canonical form is not applicable for MPDO due to its operator nature. 

Our approach is to study whether the conditional mutual information (CMI) of MPDO decays exponentially, which would then imply the existence of a parent Hamiltonian. Classically, CMI is an entropic quantity defined for probability distribution over tripartite system ABC. The smaller its CMI is, the closer they form a Markov chain. The quantum CMI and Markov chain are only defined recently, and it appears that quantum conditioning is technically much more difficult than classical. For MPDO, the logarithm featured in entropic function is difficult to calculate although the Renyi entropies are more tractable. 

We probe the CMI of a special family of MPDO constructed from sequential application of 1-input/2-output Completely-Positive map. We concretely prove the exponential decay of CMI when the repeated map is a bistochastic channel with a rate related to relative entropy. The proof idea is that the component of the density matrix contributing to tripartite entanglement shrinks at each repetition of the channel. For more general channels, we concede and conjecture a data processing inequality that the CMI must decrease with a uniform rate at each iteration of the channel. Our intuition is that a noisy local channel should uniformly shrink the entanglement with a however larger system. We also investigate the semi-classical case when the conditioned system B is projected to a measurement basis. It may be regarded as an independent problem since measurement may drastically change the CMI. We gave sufficient conditions for the exponential decay of the post measurement CMI, which are not necessary conditions, but convenient to check numerically and we believe is generic. 

Our work probes the CMI of MPDO from explicit structural decomposition of the state in a special case, a general DPI conjecture for understanding tripartite entanglement, and viewing the measured MPDO as family of Completely Positive maps and applying Hilbert’s projective metrics. We are taking the very first steps as very few properties of MPDO as well as CMI were analyzed in the literature. Some of our results are not the tightest but we regard it as pointing out inspirations for future work. 

From these reasons, we believe that the manuscript clearly meets a high criterion of Communications in Mathematical Physics. 


Yours Sincerely, 
Chi-Fang Chen, Kohtaro Kato and Fernando G. S. L. Brandão

